IO vs OI in Higher-Order Recursion Schemes

We propose a study of the modes of derivation of higher-order recursion schemes, proving that value trees obtained from schemes using innermost-outermost derivations (IO) are the same as those obtained using unrestricted derivations. Given that higher-order recursion schemes can be used as a model of functional programs, innermost-outermost derivations policy represents a theoretical view point of call by value evaluation strategy.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{D. Miller and Z. \'Esik (Eds.):  Fixed Points\\
in Computer Science 2012 (FICS 2012)\\
EPTCS 77, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.77.4}{10.4204/EPTCS.77.4}}
\pdfoutput=1

